Jamming by growth

Growth in confined spaces can drive cellular populations through a jamming transition from a fluid-like state to a solid-like state. Experiments have found that jammed budding yeast populations can build up extreme compressive pressures (over 1MPa), which in turn feed back onto cellular physiology by slowing or even stalling cell growth. Using extensive numerical simulations, we investigate how this feedback impacts the mechanical properties of model jammed cellular populations. We find that feedback directs growth toward poorly-coordinated regions, resulting in an excess number of cell-cell contacts that rigidify cell packings. Cell packings posses anomalously large shear and bulk moduli that depend sensitively on the strength of feedback. These results demonstrate that mechanical feedback on the single-cell level is a simple mechanism by which living systems can tune their population-level mechanical properties.

==> Jamming by growth - upload to arXiv/SI.tex <==
\setcounter{figure}{0}  % resets figure numbers
\renewcommand{\thefigure}{S\arabic{figure}}    % changes figure labels to S1, S2 ...
\section{Supplementary Information}

The source-codes are available on GitHub \cite{sourcecodes}.

\subsection{Cell-based simulations}\label{simmodel}
In 2D cell-based simulations, illustrated in Fig.~\ref{fig:cells}, cells are modeled as two frictionless rigidly-attached spherical lobes~\cite{schreck2010comparison,delarue2016self} (mother and bud) that grow exponentially in time at rate $\gamma_i$ by bud expansion (Eq. 1) and interact via repulsive spring forces with elastic modulus $\rm k$  (Eq. 2):

\begin{equation}\label{eq:growth}
\dot{a}_i = \gamma_i a_i
\end{equation}

\begin{equation}\label{eq:energy}
\rm V = \sum_{i>j}\sum_{k,l}\frac{1}{2} k\delta_{ik,jl}^2\Theta(\delta_{ik,jl})
\end{equation}
where $a_i=\frac{\pi}{4}(\sigma_{i,{\rm mother}}^2+\sigma_{i,{\rm bud}}^2)$ is the cell area, $\sigma_{i,\rm mother}$ ($\sigma_{i,\rm bud}$) is the diameter of the mother (bud), $\rm V$ is the total potential energy,  $\delta_{ik,jl}=\frac{1}{2}\big(\sigma_{ik}+\sigma_{jl}\big)-\big|{\bf r}_{ik}-{\bf r}_{jl}\big|$ is the overlap between lobes $k$ of cell $i$ and $l$ of cell $j$, and $\Theta$ is the Heaviside Step function (Fig.~\ref{fig:cells}). The potential energy is measured in units of $\rm k\sigma_{i,{\rm mother}}^2$ throughout this paper. 

The system is relaxed with quasistatic dynamics via conjugate gradient energy minimization \cite{press1992numerical}. Conjugate gradient minimization terminates upon one of the two conditions: (i) two successive steps j and j+1 yield nearly the same energy value $(\rm V_{j+1} - V_j) / V_j < \epsilon_{tol}^1 = 10^{-16}$ or (ii) the potential energy per particle at the current step is $\rm V_j/(kN) < \epsilon_{tol}^2 = 10^{-16}$. The forces (${\bf F}_i$) and torques ($T_i$) acting on each cell are calculated as:
\begin{equation}
{\bf F}_i=-\nabla_{{\bf r}_i} V
\end{equation}
\begin{equation}
T_i=-\partial_{\theta_i} V
\end{equation}
where ${\bf r}_i$ and $\theta_i$ are the position and orientation of cell i. For conjugate gradient minimization, we transform these forces to a $3N$-dimensional gradient of the potential energy as $\nabla V=\{F_1^x,F_1^y,\rm M_1/I_1T_1, ..., F_N^x,F_N^y,\rm M_N/I_NT_N\}$, where the ratio of moment of inertia to mass of each cell is $\rm I_i/M_i=\frac{1}{8}\sigma^2\left(\frac{1+\Delta^4}{1+\Delta^2}+2\big(\frac{(1+\Delta)\Delta}{1+\Delta^2}\big)^2\right)$ with $\Delta_i=\frac{\sigma_{i,\rm bud}}{\sigma_{i,\rm mother}}$.

In this model, all mother cells have the same size, $\sigma_{i,{\rm mother}}=\sigma$. Cells grow in a square box with periodic boundary conditions. Cell growth progresses while $\sigma_{i,{\rm bud}}<\sigma$ and culminates in division. After division, both new cells acquire a random orientation (see Fig.~\ref{fig:cells}). 

Without pressure feedback, the growth rate for cell $i$ is: $\gamma_i=\gamma_i^0$ where $\gamma_i^0$ is chosen from a uniform distribution of width $20\%$ around a mean growth rate $\gamma^0$. With pressure feedback, the growth rate is additionally exponentially modulated as $\gamma_i=\gamma_i^0e^{-P_i/P_0}$ where $P_i$ is the pressure on the bud of the cell $i$, and $P_0$ is a strength of the feedback \cite{delarue2016self}. The pressure $\rm P_i$ is calculated as $\rm P_i = \sum_{j(i)}|F_{ij}|/L_{i,bud}$, where $\rm  L_{i,bud}=\pi\sigma_{i,bud}$ is the perimeter of bud $i$, $\rm |F_{ij}|$ is the magnitude of the contact force between a bud $i$ and a particle $j$, and $\rm j(i)$ is a set of the particles in contact with $i$. In Figure~\ref{fig:K_P} we show the relation between the strength of feedback $P_0$, population-averaged growth rate $\Gamma = \frac{1}{A}\sum_i a_i\gamma_i$ ($A=\sum_ia_i$), and growth-induced pressure $P$ (see Section \ref{P_and_G} for details on the calculation of $P$).

\subsection{Generating jammed packings}
The simulation starts with two randomly oriented yeast cells. Initially the cells grow according to Equation \ref{eq:growth} with a time-step of $\rm dt_0=0.002/\gamma^0$, and this continues while $\rm V/(kN) < \epsilon_{tol}^2$. If the population energy per cell at time step $\rm j$ is greater than $\rm V_j/(kN) > 2\cdot \epsilon_{tol}^2$, the growth step is rejected and the time step is halved ($\rm dt_{j}\rightarrow \frac{1}{2}\cdot\rm dt_{j}$), and the growth step (proceeded by energy minimization) is repeated (Equation \ref{eq:growth}). If the average potential drops below $\rm V/(kN) < \epsilon_{tol}^2$, the time step is reset to $\rm dt=\rm dt_0$. The simulation terminates when the the average energy per particles of a static energy is $\rm \epsilon_{tol}^2 < V/kN < 2\cdot \epsilon_{tol}^2$. 

This growth-driven protocol differs from previously-used compression protocols~\cite{olafsen2010experimental}. Whereas compression simulations start with a fixed number of objects and reduce the box size until the systems jams, growth-driven simulations start with few objects and increase the number of objects via growth until the system jams. 

Once the population reaches the jamming point at $\phi_J$, the colony grows beyond that point\textemdash up to the preassigned value $\delta \phi = \phi-\phi_J$. The protocol is similar to the one used to find $\phi_J$, however the time-step is halved when the volume fraction exceeds $\delta \phi$ by a margin of $\Delta=0.5\cdot 10^{-8}$, i.e. $\phi > \phi_J + \delta \phi + \Delta$. The time-step is reset to $dt=dt_0$ if the volume fraction falls below: $\phi < \phi_J + \delta \phi - \Delta$. The protocol ends when the volume fraction falls into the range $\phi \in \left[\phi_J + \delta\phi - \Delta , \phi_J+\delta\phi + \Delta \right]$.

To speed up simulations where population pressure significantly slows down growth ($P\gg P_0$), we use an adaptive time-step. In this method, we scale the time-step $dt$ by the largest cellular growth-rate in the population $\gamma_{\rm min}$: $dt'=dt\cdot \gamma/\gamma_{\rm min}$. This method ensures that, even while the population is under pressure, the fastest-growing cells add the same amount of volume per time-step as they would have without feedback. Unless noted explicitly, all results in this paper use this adaptive time-step method. 

\subsection{Calculation of mechanical properties}\label{P_and_G}

For each static packing, we calculate the stress tensor $\hat{\Sigma}$ via the Virial expression:
\begin{equation}
\rm \hat{\Sigma}_{\alpha\beta} = \frac{1}{2L^2}\sum_{i>j}\sum_{k,l}\big(r_{ik,jl}^\alpha F_{ik,jl}^\beta+r_{ik,jl}^\beta F_{ik,jl}^\alpha\big)
\end{equation}
where $\rm F_{ik,jlj}^\alpha$ is the $\alpha$-component of the force $\vec{F}_{ik,jl}$ on $k$th lobe of particle $i$ resulting from overlap with the $l$th lobe of particle $j$, and $\rm r_{ik,jl}^\alpha$ is the  $\alpha$-component of the vector from the center of mass of lobe $ik$ to the center of mass of lobe $jl$. The pressure is calculated from the stress tensor as $\rm P=\frac{1}{2}\big(\rm \hat{\Sigma}_{xx}+\rm \hat{\Sigma}_{yy}\big)$.

To calculate bulk modulus B, the simulation box is compressed by $d\phi=10^{-8}$, and the modulus is calculated from the definition $B=\phi dP/d\phi$.

To determine shear modulus G of a cellular packing, the response to quasistatic simple shear is calculated. To that end, for a static packing at $\delta \phi = \phi - \phi_j$, each cell is subject to a small affine shear strain (along the x direction with gradient in the y direction):
\begin{equation}
\rm x_i \rightarrow x_i + \delta\gamma y_i
\end{equation}
where $\rm \mathbf{r}_i = (x_i,y_i)$  is the location of the center of mass of a particle $i$, and $\delta \gamma = \delta x/L = 10^{-6}$, and $L$ is size of the system. Following the application of shear strain, the system is relaxed via energy minimization. Then, shear modulus is calculated from the definition $G=d\Sigma_{xy}/d\gamma$.

Throughout this paper we measure $P$, $B$, and $G$ in units of the cell-cell modulus $\rm k$.

\subsection{Pressure scale ($P_{\rm max}$) at confluency ($\phi=1$)}
\label{appx:pmax}

Population pressure $\rm P$ is determined by the overlap between cells, which in turn is set the compression beyond the jamming point $\delta\phi=\phi-\phi_J$. Here, we estimate the pressure $P_{\rm max}$ resulting from compression of cell packings from jamming $\phi_J=0.84$ to confluency $\phi=1$. 

By explicitly calculating the force between lobes $ik$ and $jl$, $F_{ik,jl}^\alpha=-\partial_{r_{ik}^\alpha}V=r_{ik,jl}^{\alpha}/r_{ik,jl}\times k\delta_{ik,jl}$, we can reduce the population pressure to $P=\frac{1}{2L^2}\sum_{i>j}\sum_{kl}kr_{ik,jl}\delta_{ik,jl}$. This can be expressed as an average over the $N_c=Nz/2$ contacts in the system, so that $P=\frac{Nz}{4L^2}\langle k r_{ik,jl}\delta_{ik,jl}\rangle$.

To estimate $P$, we assume that we have a population of monodisperse spherical cells with diameter $\sigma$ with $z\approx z_J=4$ and $\phi_J=0.84$. Further assuming that cells compress purely affinely upon infinitesimal compression, equivalent to swelling cells from $\sigma$ to $\sigma+d\sigma$ while keeping the box size fixed at $L$, and that no new contacts are made in the process allows us to simplify pressure to $P=\frac{N}{L^2}k\sigma d\sigma$. Since the volume fraction is $\phi=\frac{N\pi\sigma^2}{4L^2}$, $d\phi=\frac{N\pi\sigma}{2L^2}d\sigma$ and $\frac{N}{L^2}\sigma d\sigma=\frac{2}{\pi}d\phi$. This allows us to relate $P$ to changes in $\phi$: $P/k=\frac{2}{\pi}d\phi$.

Finally, we are able to calculated the pressure $P_{\rm max}/k=\frac{2}{\pi}0.16\approx 0.1$ generated by compressing a cell paacking from $\phi_J=0.84$ to $\phi=1$. This value is consistent with our measured data in Fig.~\ref{fig:sims}g.

\subsection{Modified isostaticity at jamming point}\label{appx:z-iso}

In this section we describe why the ``isostatic'' criterion for growing budding cells differs from the naive expectation of $Z_{\rm iso}^{\rm naive}=6$. 

In order for a system to be mechanically-stable, it must have as many contacts in the system ($N_c$) as degrees of freedom ($N_d$). This is the naive isostatic, or Maxwell, criterion. Since budding cells have $3$ degrees of freedom per cell, the system has a total of $N_d=3N$ degrees of freedom and we would naively expect there to be be $N_c=N_d=3N$ degrees of freedom at jamming, or $Z_{\rm iso}^{\rm naive}=2N_c/N=6$ contacts per cell. This argument breaks down, however, because not all degrees of freedom in the system are constrained. Unconstrained buds and rattlers decrease the contact number at jamming $Z_J$ below $Z_{\rm iso}^{\rm naive}=6$ because contacts are not required to constrain these degrees of freedom. The isostatic criterion, taking into account unconstrained buds and floaters, is $N_c^{\rm iso}=3N-3N_r-N_u-1$ where $N_r$ and $N_u$ are the number of rattlers and unconstrained buds in the system and the $-1$ is a finite-size correction.  We can express the isostatic criterion as $Z_{\rm iso}=2N_c^{\rm iso}/(N-N_r)=6-2f_u-2/(N-N_r)$ contact per (non-rattler) cell, where $f_u$ is the fraction of (non-rattler) cells with an unconstrained bud. Fig.~\ref{fig:Z_iso} shows that this isostacity criterion holds for nearly all packings analyzed. Note that in the main text we use the large-system limit $Z_{\rm iso}\big|_{N\rightarrow\infty}=6-2f_u$ and in Fig.~\ref{fig:Z_iso} we take into account finite-size effect by adding $2/(N-N_r)$ to $Z_J$ \cite{goodrich2012}. 

\subsection{Hyperstaticity due to unconstrained bud growth}
\label{appx:z-hyper}

In this section we describe why growth under extreme feedback produces ``hyperstatic'' ($Z>Z_{\rm iso}$) packings. In the case of extreme feedback ($P_0\rightarrow 0$), only unconstrained buds grow above the jamming point and these buds cease growing once they come into contact with their neighbors. If there are $N_u=f_uN$ unconstrained buds at jamming and of these $\Delta N_u=\Delta f_uN$ have come into contact with their neighbors due to growth above jamming, then the population needs $Z_{\rm iso}=2(3N-N_u+\Delta N_u)/N=6-2f_u+2\Delta f_u$ contacts for mechanical stability. However, each new unconstrained bud needs $2$ contacts to stabilize it, so that the contact number increases to $Z=2(3N-N_u+2\Delta N_u)/N=6-2f_u+4\Delta f_u$ as unconstrained buds make contact. So, as unconstrained buds make contact the system become hyperstatic with $\Delta Z'=Z-Z_{\rm iso}=2\Delta f_u$. In the extreme case, $\Delta Z'=2f_u$ is determined by the number of buds that were unconstrained at jamming. Note that this deviation from isostaicity is twice as large as the deviation from the coordination number at jamming, $\Delta Z=Z-Z_J=4\Delta f_u$, which we show in the paper.  

\begin{figure*}
\includegraphics[width=\textwidth,keepaspectratio]{./Figures/sim_schematic_v3.pdf}
\caption{
Schematic of (a) the growth and (b) division processes and (c) cell-cell interactions in our cell-based simulations. Each cell is composed to two lobes, the mother (gray) and bud (yellow). (a) During growth, the mother lobe diameter of cell $i$ stays fixed at $\sigma_{i,{\rm mother}}=\sigma$ while the bud grows from $\sigma_{i,{\rm bud}}=0$ to $\sigma_{i,{\rm mother}}=\sigma$. (b) Once the bud reaches $\sigma_{i,{\rm mother}}=\sigma$, cell $i$ divides into two new daughter cells that have random orientations. (c) Cells $i$ and $j$ interact only upon overlap ($\delta_{ik,jl}$) via repulsive linear spring interactions with modulus $\rm k$.}
\label{fig:cells}
\end{figure*}

\begin{figure*}
\includegraphics[width=\textwidth,keepaspectratio]{./Figures/Z_iso_fu.png}
\caption{
Average number of contacts $\rm Z_J$ as a function of a fraction of unconstrained buds $\rm f_{\rm u}$. Dashed-line gives the relation $Z_{\rm iso}=6-2f_u$ from constraint counting arguments. A small correction $2/\left<N\right>$ has been added to $\rm Z_J$ to account finite-size effects (Section \ref{appx:z-iso}).
All simulated packings have at least as many contacts as expected ($\rm Z_J\geq Z_{\rm iso}$) while the majority of packings exactly satisfy $\rm Z_J=Z_{\rm iso}$. Numerical data is shown for system sizes $\left<N\right>=75$,$\left<N\right>=172$ $\left<N\right>=307$.}
\label{fig:Z_iso}
\end{figure*}

\begin{figure*}
\includegraphics[width=\textwidth,keepaspectratio]{./Figures/B_dPhi_linear.png}
\caption{
Bulk modulus as a function of volume fraction above jamming $\delta\phi=\phi-\phi_J$ for populations growing under five different feedback strengths. 
}
\label{fig:B_dPhi_linear}
\end{figure*}

\begin{figure*}
\includegraphics[width=\textwidth,keepaspectratio]{./Figures/B_dZ_linear.png}
\caption{
Bulk modulus as a function of number of  cell-cell contacts above jamming $\Delta Z=Z-Z_J$ for populations growing under five different feedback strengths. 
}
\label{fig:B_dZ_linear}
\end{figure*}

\begin{figure*}
\includegraphics[width=0.95\textwidth,keepaspectratio]{./Figures/K_P_relabel.pdf}
\caption{Population-averaged growth rate $\Gamma$ as a function of the population averaged pressure $P$. $\Gamma$ is calculated from individual cell growth rates $\gamma_i$ as $\Gamma=1/A\sum_{i}\gamma(i)A(i)$, where $A(i)$ is the area of the $i^{th}$ cell, $\gamma(i)$ is the growth rate of the $i^{th}$ cell (at a given time-step), and $A = \sum_{i}A(i)$. Population-averaged pressure is calculated form the stress tensor $\Sigma_{\alpha\beta}$ (see Section \ref{P_and_G} for details). The results are for 6 different strengths of feedback: No feedback (green), $P_0=10^{-2}$(cyan), $P_0=5\cdot 10^{-3}$(dark blue), $P_0=10^{-3}$(blue), $P_0=5\cdot 10^{-4}$(purple), and $P_0=10^{-4}$ (red). Dashed-lines are fits to the numerical data. Fitted feedback strengths are given of the right-hand side of the legend. Simulations were done with time-steps kept constant, without the adaptive time-steps method. }
\label{fig:K_P}
\end{figure*}
